Understanding Reasoning in Chain-of-Thought from the Hopfieldian View

Large Language Models have demonstrated remarkable abilities across various tasks, with Chain-of-Thought (CoT) prompting emerging as a key technique to enhance reasoning capabilities. However, existing research primarily focuses on improving performance, lacking a comprehensive framework to explain and understand the fundamental factors behind CoT's success. To bridge this gap, we introduce a novel perspective grounded in the Hopfieldian view of cognition in cognitive neuroscience. We establish a connection between CoT reasoning and key cognitive elements such as stimuli, actions, neural populations, and representation spaces. From our view, we can understand the reasoning process as the movement between these representation spaces. Building on this insight, we develop a method for localizing reasoning errors in the response of CoTs. Moreover, we propose the Representation-of-Thought (RoT) framework, which leverages the robustness of low-dimensional representation spaces to enhance the robustness of the reasoning process in CoTs. Experimental results demonstrate that RoT improves the robustness and interpretability of CoT reasoning while offering fine-grained control over the reasoning process.

==> old_version/3_preliminary_v9_16.tex <==
\section{Preliminaries}

\subsection{Representations in Large Language Models Reasoning}

Prompts can be designed to guide large language models to solve problems more effectively by instructing them to provide a series of intermediate reasoning steps leading to the final answer. \citet{wei2022chain} demonstrated that a large language model denoted as $M_\theta$ parameterized by $\theta$ \di{add a paragraph on LLM in the Preliminary section}, can generate chains of thought when few-shot demonstrations $D = (q_1,a_1; q_2,a_2; ...)$ are provided in their context window \di{what are $q_1$...?}.
Additionally, \citet{kojima2022large} demonstrate the potential of large language models to act as zero-shot reasoners, capable of following an instruction $I$ like ``let's think step by step" to provide more reasoning steps before arriving at the final answer. 


The existing literature has shown that when LLMs receive these task-specific instructions or a series of demonstrations, an emergent and semantically meaningful internal structure can be observed within neural networks~\citep{zou2023representation}. This internal structure may manifest as task vectors, which can be modified and combined with the model’s parameters \citep{ilharcoediting,ortiz2024task}. Additionally, representations can be formed by summing the outputs of the causal attention heads in LLMs and incorporating this representation vector into the model's hidden states as it processes a prompt, thereby controlling the model's behavior~\citep{ilharco2022editing} \di{This sentence needs some details and hard to understand}.  \di{I think the above sentences should be moved to preliminaries. }


==> old_version/4_experiment_copy.tex <==
% \input{tables/main_result}
\input{tables/arithmetic_reasoning_result_table}
\input{tables/commonsense_reasoning_result_table}
\input{tables/symbolic_reasoning_result}


\subsection{Utility Evaluation}

In this section, we use the reading vector $v$ to control the generation of CoT reasoning paths. As shown in Table~\ref{tab:arithmetic_result},~\ref{tab:commonsense_result} and~\ref{tab:symbolic_result},
we present the performance comparison between our approach and baselines on each task. From these tables, we can see the following interesting findings.

\paragraph{(i) Our framework can guide/correct the reasoning direction of LLM.}
% \warn{FIX-XIN: change a title - Enhanced rReasoning aAccuracy in both few-shot and zero-shot CoT. Using Our Approach in Zero-Shot and Few-Shot CoT Scenarios}
For example, for zero-shot CoT, our approach demonstrates superior performance, surpassing Mistral-7B-instruct by 4\% on the SVAMP dataset, and for few-shot CoT, our approach achieves a significant improvement over LLaMA-2-7B-chat by 2.95\% on the CSQA dataset. This is mainly because our approach demonstrates that our methodology effectively directs the correct reasoning path of LLM, thereby improving the accuracy of reasoning. This highlights the effectiveness our interpretability in CoT, which employs concept-level representation read operations to localize errors in CoT, followed by control operations to rectify LLMs’ reasoning paths.

% \paragraph{(ii) Few-shot CoT simply activates the LLM concept of answer style. \warn{FIX-XIN: need to change a title - Few-Shot Learning Leads to Stereotyped Reasoning Compared to Zero-Shot Control}} 
\paragraph{(ii) Few-shot CoT have stereotypes in the reasoning phase.}

From these tables, we observe that, except for the commonsense reasoning task, our approach generally performs better on zero-shot control than con few-shot control. This is mainly due to the fact that it is affected by the few shot examples. 
To investigate why the performance of the few-shot concept is inferior to that of the zero-shot prompt, we analyzed instances where the few-shot CoT concept failed. As illustrated in Figure ~\ref{fig:zero_few_control}, it shows that the model answered incorrectly in the red part by the few-shots learning while initially stating a correct fact of the question in the blue part. It was affected by the few shots that someone even flipped the coin. Afterward, this behavior reinforces the incorrect cognition by adding the few-shots control that the model is wrong initially stating a fact. After adding the zero-shot control, the model accurately answered the question by stating the correct facts. These results indicate that few-shot learning produces the stereotype when reasoning.

\eat{The results also show that the few-shots concept is inferior to the zero-shot concept in arithmetic Reasoning and symbolic reasoning, although few-shots perform well in commonsense reasoning. 
To investigate why the performance of the few-shot concept is inferior to that of the zero-shot prompt, we analyzed instances where the few-shot CoT concept failed, as illustrated in Figure ~\ref{fig:zero_few_control}. The figure shows that the model answered incorrectly in the red part by the few-shots learning while initially stating a correct fact of the question in the blue part. It was affected by the few shots that someone even flipped the coin. Afterwards, this behaviour reinforces the incorrect cognition by adding the few-shots control that the model is wrong initially stating a fact. After adding the zero-shot control, the model accurately answered the question by stating the correct facts. These results indicate that few-shot learning produces the stereotype when reasoning. }

\eat{
1) our approach can guide/correct the reasoning direction of LLM, thereby improving the accuracy of reasoning.
2) zero-shot CoT stimulated by prompt (\emph{``Let's think step by step''}) can activate the reasoning concept of LLM.
3) few-shot CoT, especially when only a few examples are given, simply activates the LLM concept of answer style.
}


% \warn{
% Meanwhile, we can observe that the LLaMA-3 model zero-shot CoT can beat the few-shot CoT on most dataset benchmarks. The reason for this is that LLaMA-3 is trained on more than 15T tokens and internalizes the reasoning process.
% }

\subsection{Read Process Interpretability}
To further demonstrate the effectiveness of our approach, we provide additional cases in three models on arithmetic, commonsense, and symbolic reasoning tasks in Appendix \ref{Appendix:case_demo} (See Figure \ref{fig:case_aqua_zero}, \ref{fig:case_strategyqa_few}, \ref{fig:few_shot_case_llama3_coin_flip}, and \ref{fig:coterrorexample}).

For zero-shot CoT, Figure~\ref{fig:case_aqua_zero} displays the real prediction of a case by the model both without control and control. 
From this figure, we can observe that the model is wrong when simplifying the equation, and the reasoning path is offset. As shown in the \textcolor{crimson}{red} part, the reason for the mistake of the model is that multiple steps have been performed in the process of simplification, which leads to calculation errors.
After adding control to the model, the direction of the reasoning path of the model will be corrected to achieve the calculation error that occurs when the control is not added.

For few-shots CoT, Figure~\ref{fig:case_strategyqa_few} demonstrates the real prediction of a case by the model both without control and with control on the strategyQA dataset. From this figure, we can observe that the model initially makes a correct inference regarding the elevation of Mount Fuji and the depth of the Sea of Japan. However, the model erroneously concludes that Mount Fuji would not be out of the sea due to a miscalculation in comparing the mountain’s height with the sea’s depth as illustrated in the \textcolor{crimson}{red} segment. After adding control to the model, the reasoning path leads to the correct conclusion that the top of Mount Fuji would indeed be out of the Sea of Japan, as highlighted in the \textcolor{seagreen}{green} segment. 

The results highlight our interpretability in CoT, which employs concept-level representation read operations to localize errors in CoT, followed by control operations to rectify LLMs’ reasoning paths. This intuitive interpretable analysis for CoT reasoning is helpful in tracing and controlling the errors LLMs made during the CoT process.


\subsection{Control Process Interpretability}


\subsection{Ablation Study}



\eat{
\warn{FIXXIN: why are there two similar case here?} Additionally, Figure~\ref{fig:few_shot_case_llama3_coin_flip} also showcases that the model initially makes a correct inference step by step about the coin's state after each flip.  However, the error arises from not correctly accounting for the even number of flips by Kydin. After adding control, the model correctly reasons that the coin has flipped a total of two times, an even number, leading to the accurate conclusion that the coin remains heads up, as shown in the \textcolor{seagreen}{green} segment. These demonstrate the significance of control in ensuring the model follows the correct reasoning path.
}


==> old_version/4a_explanation_framework.tex <==
\section{CoT Explanation from Hopfieldian View}
\syinline{need to be rewrite}

\label{sec:method}

In this section, we will dive into details about our motivation from the  Hopfieldian view and a general introduction of our framework. 


%In this section, we first describe our interpretability framework, and then we present our approach to validating it. Finally, we describe how this framework can be used to improve the CoT capability of LLMs.

\noindent{\bf Motivation.}
Existing literature has confirmed that CoT can improve the reasoning ability of LLMs~\cite{kojima2022large,wei2022chain}. 
However, few studies have conducted a comprehensive analysis of the interpretability of CoT. 
This is mainly because reasoning is a complex task, and the model's final performance is influenced by numerous factors. 
Analyzing internal activations in isolation or from the perspective of individual neurons of LLMs is challenging. 
Inspired by work related to representation engineering~\cite{zou2023representation}, we consider LLM from a higher-level cognition perspective (Hopfieldian view), \ie specific external stimuli activate representations within the model, thereby causing the model to exhibit different behaviors that represent the population activation behavior of neurons within the model.
Meanwhile, many studies have shown that the representations of LLM are almost secretly linear inside, and can be controlled via linear probe methods~\cite{Park2023linearhp,wu2024reft}.
These phenomena indicate that we can analyze the interpretability of CoT from the perspective of representation and control the reasoning process of LLM.

\input{tables/fig1}

\eat{
LLM learned latent (both concrete and abstract) concepts from pertaining documents. 
These concepts might pertain to specific names or domains, such as ``medical'' or ``climate change''. 
They could also represent more abstract notions derived from document-level modeling, such as ``positive language'', ``careful reasoning'', or ``affirmative expression''. 
During the reasoning process, zero-shot or few-shot prompts serve as stimuli for the LLM, inducing the activation of specific concepts. 
These activated concepts collectively determine the final action of this model.
However, directly extracting activated concepts would consume a tremendous amount of computational resources, and individual concepts alone cannot determine the model's overall action. 
Therefore, we use representations to denote the activation of concepts when the model is stimulated.
}

\noindent{\bf Framework.}
As we are targeting at exploiting the Hopfieldian view to provide an explanation for LLMs' CoT reasoning, we have to build a bridge from the components in the cognitive brain to CoTs. We begin from introducing the definition of stimulus in CoT, which is the prompt text (\ie example input-output demonstrations in a few-shot scenario and \emph{``think step by step''} in a zero-shot scenario). Then use these stimuli to activate specific "neural populations" for CoT.


For neural populations, ideally, we can leverage humanly comprehensible concepts within LLMs' representations. To model these concepts, our framework has two phases: 
(i) \emph{Concept Modeling},  and (ii) \emph{Concept Simulation}. 
In the Concept Modeling phase (Section \ref{sec:stage1}), LLMs will learn latent (both concrete and abstract) concepts from pertaining documents, and these concepts might pertain to specific names or domains, such as ``medical'' or ``climate change''. 
They could also represent more abstract notions derived from document-level modeling, such as ``positive language'', ``careful reasoning'', or ``affirmative expression''. 
Likewise, in the Concept Simulation stage (Section \ref{sec:stage2}), zero-shot or few-shot prompts serve as stimuli for the LLM, inducing the activation of specific concepts. 
These activated concepts collectively determine the final action of this model.

However, directly extracting activated concepts would consume a tremendous amount of computational resources, and individual concepts alone cannot determine the model's overall action. 
Therefore, our framework uses representations to denote the activation of concepts when the model is stimulated. 
For this, our framework employs \emph{Representations  Reading} (Section \ref{sec:stage3}) and \emph{Representations Controlling} (Section \ref{sec:stage4}) as the core modeling components.  

Next, we will give details about the individual model components. Later, we explain how this framework can be used to improve the CoT reasoning abilities of LLMs. See Figure \ref{fig:framework} for an illustration of our framework.  
%This work exploits Hopfieldian view to provide an explanation for LLMs' CoT reasoning by leveraging  humanly comprehensible concepts within LLMs' representations. 
%The core components of our model are as follows: Documents Modeling, Concept Stimulation, Reading Representations, and Controlling Representations.


\section{Details of the Framework}

\liang{Reviewer: Section 5 is subdivided again and again into numerous subsections, drawing attention to the intricacy and the number of moving parts required in trying to apply this novel techniques. Yet there are few experiments in that section that justy the paper's design choices in each of the possible moving parts. }

\mlinline{I think we need to rewrite this section to highlight the challenges and our contributions in the methodology. }

\subsection{Concept Modeling}\label{sec:stage1}
Previous research~\cite{xie2021explanation} reveals that during pre-training LLMs can learn a set of latent document-level concepts $c \in C$ that in turn help large language models to generate coherent next tokens. 
This motivates our design of stimuli. 
We provide some examples of these concepts in Figure~\ref{fig:framework}.
The activation and intensity of specific concepts determine the model's final response. 
However, searching and controlling individual concepts is a prohibitively expensive process. 
In order to circumvent that, we instead use representations as a basic unit indicative of latent concepts learned by the model.
We cover the definitions and relationships between these representations and concepts in the next subsections.

% \begin{equation}
% \mathbb{P}(r | p) = \mathbb{P} (r | Rep([\mathcal{S}, x])) 
% \end{equation} \\

% \syinline{As a reader, I still do not understand what is the stimulus $S$ in LLMs. You should give more details in the motivation section 4.1. Also, why introduce Rep? And what are the details of Rep?}
% \syinline{How do you get these c? Need more details!} 

%\noindent{\bf Modeling Concepts from Documents.}


\subsection{Concept Stimulation}\label{sec:stage2}
\warn{
From the Hopfield view, we need specific stimulus to trigger the model's specific action. 
Since CoT reasoning is primarily activated through prompts, we posit that CoT prompts $p$ containing a set of stimulus $S$ that can activate the model's reasoning capabilities. 
So, we use the following formula based on Bayesian inference to illustrate the entire process from the LLM receiving an input to generating a specified output, as shown in Figure~\ref{fig:framework}:
\begin{equation}
\label{eq:bayes_2}
\mathbb{P}(r | p) =  \int_{c} \mathbb{P} (r |c,T([\mathcal{S}, x]))  \mathbb{P} (c | T([\mathcal{S}, x])) \mathop{d}(c),
\end{equation}
where, $T([S, x])$ is the prompt template based on specific Stimulus $S$ and query $x$. 
$\mathbb{P} (r |c,T([\mathcal{S}, x]))$ is the likelihood of response $r$ given $c$, 
and $\mathbb{P} (c | T([\mathcal{S}, x]))$ is the prior
probability of the $c$ for a given prompt template
$T([\mathcal{S}, x])$.
}

This equation governs the conditional probability of a response $r$ given prompt $p$ guided by concept 
\emph{i.e.,} $(c \in C)$ learned by the model. 

%\eat{\paragraph{Representations: \warn{readable} and controllable units in LLMs}}
%\noindent{\bf Reading and Controlling Representations.} 

% \warn{Liang: Decribe Equation here briefly...!}
% \fixli{Plz briefly describe above eq here..!} it's clear enough

\subsection{Representations Reading}\label{sec:stage3}
The end goal of reading representations is to look
for and/or locate the representations for key 
concepts within a network.
We sub-divided its process into: 
(a) concepts reading, and 
(b) reasoning error localization. 
Details about each component are explained in the following sub-sections.

\eat{
\subsubsection{Stimuli Selection}
\label{sec:select_stimuli}

To elucidate the sensitivity of LLMs to different CoT prompts, we employ various ``\emph{stimuli}'' encompassing one or more concepts for inducing diverse model behaviors under both zero-shot and few-shot settings. Our objective is to analyze how the concepts corresponding to a specific stimulus are processed and transferred within large models, as illustrated in Figure~\ref{fig:hopfieldianandstumili}, from the perspective of cognitive neuroscience.

We  explain the impact of stimulus in Hopfieldian 
view as follows: \liang{given a set of stimuli (i.e., the prompt text) $S = \{s_{0}^{-}, s_{0}^{+}, s_{1}^{-}, s_{1}^{+}, \cdots, s_{n}^{+}\}$,} when an LLM receives a positive stimulus 
$s^+$, it generates a specific output/response $r$, across 
a query $x$, and falls into the corresponding action 
space $A^+$. 
Conversely, when it receives a negative stimulus $s^-$ or no stimulus at all, the model's output falls into a different action space $A^-$ or $A$.

For this, we aim to analyze, why providing 
examples can improve the reasoning accuracy of LLMs. 
An example of a pair of specific prompt template for
$T([\mathcal{S}, x]))$, and example demonstrations 
for few-shot CoT are shown in Appendix~\ref{Appendix:prompts}.

\di{I cannot see any method in this subsection, why you make it as a step? I think you should merge with Sec. 5.3.2. or put it at the beginning of section 5.3}
}


% \fixli{I think some stimuli-specific examples will help here..!}
% \fixshu{What are negative and positive examples + why we need them..? Clarify with example}


% need to rewrite
\eat{
\subsection{Rationale Generation}
\label{sec:BRG}
The core objective of the \warn{rationale} generation 
is to prompt the LLM using a CoT prompt in order to 
come up with a \warn{rationale} path. This process is illustrated 
in step-\warn{2} of the Figure~\ref{fig:framework}.
Formally, given a large model 
$\mathcal{M}_\theta$ parameterized by $\theta$, we 
generate a \warn{rationale $R$} as follows:
\begin{equation}
    \mathcal{F}: (Q, t) \rightarrow R
\end{equation}
where $\mathcal{F(\cdot)}$ is the function primarily 
powered by the model $\mathcal{M}_{\theta}$, 
\eat{$Q$ is the complex question,} 
and $t$ is the special text added to the prompt.
}


\eat{
a base reasoning path $R$ is generated by .
Step 1 in Figure~\ref{fig:framework} illustrates how 
we generate a base reasoning path $R$: given a complex 
question $Q$, a base reasoning path $R$ is generated 
by LLM $\mathcal{M}_\theta$. It can be defined as:}


\subsubsection{Concepts Reading}
\label{sec:reading}
This module aims to locate and highlight the core concepts within the network. 
The concepts output/generated by this module act as a foundation for the subsequent steps, \ie representation evaluation followed by representation control.
However, in CoT-style prompting, the definition of concepts is abstract, and how to define high-level concepts is crucial.
For this, we utilize a Linear Artificial Tomography (LAT), 
similar to \cite{zou2023representation}, in order to 
identify the directions of the key concept, as illustrated 
in Algorithm~\ref{alg:LAT}.
It encompasses two \mlinline{Should be three?} different modules:
(i) Stimuli Selection; 
(ii) Neural Activity Monitoring; and
(iii) Concept Identification, with each module 
explained as follows: 
\mlinline{We should make it clear which part is novel and which part is from \cite{zou2023representation} in the methodology of ``Concepts Reading''. It seems that Algorithm 1 is an existing method.}

\input{tables/LAT_algo}

\input{tables/control_ag}


% \paragraph{(i) \warn{Task}-specific Stimulus Prompting.}
% The end-goal of task-specific stimulus prompting is 
% to explicate different neural activities and functions 
% helpful for identifying CoT-related key concepts ($c$).
% In order to capture the concept $c$, in this paper,
% we design different prompt text as stimulus for 
% zero-shot and few-shot CoT respectively.

% Specifically, for zero-shot CoT, we append the text 
% "\emph{Let's think step by step}" as a prompt 
% prefix~\cite{kojima2022large}. 
% This intends to explore how in zero-shot CoT 
% this prompt prefix impacts the reasoning ability 
% of LLMs.
% For few-shot CoT, we use $n$ different example 
% demonstrations~\cite{wei2022chain} prior to 
% generating response from LLM.
% For this, we aim to analyze, why providing 
% examples can improve the reasoning accuracy of LLMs. 
% An example illustration of pair of positive and 
% negative prompt templates is given in 
% Appendix~\ref{Appendix:Prompts_T} 
% (Table~\ref{tab:prompt_for_stimulus}).
% \fixli{Why we need negative pairs as well..?}


% \warn{Also look at the 3.1.1 step-1 in RePE paper 
% to see what exactly we need to capture for the CoT task}
% \fixli{Current detail is not sufficient.}


% \pagebreak

\input{tables/reading_case}

\paragraph{(i) Stimuli Selection.}
\label{sec:select_stimuli}

To elucidate the sensitivity of LLMs to different CoT prompts, in this step we will employ various ``\emph{stimuli}'' encompassing one or more concepts for inducing diverse model behaviors under both zero-shot and few-shot settings. 
Our objective is to analyze how the concepts corresponding to a specific stimulus are processed and transferred within large models, as illustrated in Figure~\ref{fig:hopfieldianandstumili}, from the perspective of cognitive neuroscience.

We implement the impact of stimulus in Hopfieldian 
view as follows: a set of stimuli (\ie the prompt text) $S = \{s_{0}^{-}, s_{0}^{+}, s_{1}^{-}, s_{1}^{+}, \cdots, s_{n}^{+}\}$, when an LLM receives a positive stimulus 
$s^+$, it generates a specific output/response $r$, across 
a query $x$, and falls into the corresponding action 
space $A^+$. 
Conversely, when it receives a negative stimulus $s^-$ or no stimulus at all, the model's output falls into a different action space $A^-$ or $A$.

\eat{
For this, we aim to analyze, why providing 
examples or a prompt text (\ie ``Let's think step by step'') can improve the reasoning accuracy of LLMs.
}

An example of a pair of specific prompt template for $T([\mathcal{S}, x]))$, and example demonstrations are shown in Appendix~\ref{Appendix:prompts}.

\paragraph{(ii) Neural Activity Monitoring.}
After receiving the task-specific prompt stimuli set, 
the next step is to capture corresponding representations 
from the LLM. 
Given that LLMs rely on transformer-based architecture to store distinct representations intended for different purposes. 
In order to capture the representations for the specific 
task, we first need to identify suitable design choices for the extraction process.
For decoder-only/auto-regressive architecture models, one 
natural choice is to choose the position of the \emph{last token} as the representation of each concept. 

Formally, given a set of stimuli $S$, a language model $\mathcal{M}_{\theta}$, and a function $\text{Rep}$,  we compute the neural activity $A_c$ as follows:
\begin{equation}
\label{Eq:NA}
    A_c = \{\text{Rep}(s_i, \mathcal{M}_\theta)[-1] \;|\; s_i \in S \},
\end{equation}
where $\text{Rep(.,.)}$ is a function that takes stimulus $s_i \in S$ and LLM $\mathcal{M}_{\theta}$ as input and returns the representations from all token positions. 
% $\text{Rep(.,.)[-1]}$ takes stimulus $s_i \in S$ and LLM $\mathcal{M}_{\theta}$ as input and returns the representations corresponding to its last token. 
% \di{What is [-1]? Why you need this? }


\paragraph{(iii) Concept Identification.}\label{subsec:vector}
Concept identification aims to identify a direction that accurately predicts the underlying concept solely based on the neural activity recorded via~\eqref{Eq:NA}.

\liang{Reviewer: Why should one take the difference of representations (I am assuming they are the residual stream activations) and compute PCA? How is this related to the latent concept?}

\eat{
For this, we employ Principal Component Analysis (PCA)  to the set of difference vectors that can yield superior results when the stimuli in each pair share similarities except for the target concept.
}
\warn{
For this, as \citet{zou2023representation} have suggested, we employ Principal Component Analysis (PCA) in an unsupervised manner, and use the set of difference vectors as inputs. It can yield superior results when the stimuli in each pair share similarities except for the target concept.
}


Specifically, we compute the principal components of the representation $\{ A_{c}^{i+1} - A_{c}^{i} \}$ (as depicted in line~\ref{line:diff} of Algorithm~\ref{alg:LAT}),
and define the leading principal vector derived 
from this as ``reading vector'', denoted by $v$.
Intuitively, we can compute the dot product between the 
reading vector $v$ and each representation $\text{Rep}(s_i, \mathcal{M}_\theta)$ as an indicator of the relevance 
between the stimulus representation and latent concepts.


%Monosemanticity aims to enhance interpretability by ensuring that each feature uniquely corresponds to a specific concept within the LLM, thereby facilitating a clearer understanding of how intermediate activations contribute to the model's predictions.  \di{No, this pagragraph should not be here. 



\subsubsection{Reasoning Error Localization}
\label{sec:EV}

% When we capture the reading vector $v$ about concept $c$, 

In this section, we consider the visualization of reasoning error localization, 
given a query $x$, we format it using the stimulus prompting template $T$ and represent it as $p$. Then, we use $p$ to generate a base reasoning path $R$ with $\mathcal{M}_\theta$.
% \di{Why we need to consider evalaution? What is the goal of this step? I do not understand! }
% Followed by utilizing a procedure akin to Section~\ref{sec:reading} to acquire the representations $H$, and these values of $H$ are then normalized using the parameters derived during the construction of the PCA model in the training phase. 
% We first utilize the LLM to generate the base reasoning path 
% $R$ \di{If you donot want give details here, just add refence.}, followed by utilizing a procedure akin to Section~\ref{sec:reading} to acquire the representations $H$ \di{You did not use H in the following part!}.
% These representations are normalized leveraging the parameters derived during the construction of the PCA model in the training phase \di{I don't understand, why these representations? Also what is normaled....}

After the representations reading (section~\ref{sec:reading}), we get the reading vector $v$.
Then, we compute the dot product between the representations $\text{Rep}(p,\mathcal{M}_\theta)$ and our reading vector $v$ yielding
a set of scores, which serve as the basis for reasoning error localization. We use the score of each token compared against a threshold $\delta$ to locate errors in the reasoning path.
Specifically, we use the following criterion to access and/or evaluate the quality of the rationales:
\begin{equation}
    \text{scores}_{norm} = 
    \text{normalize}(\text{Rep}(R, \mathcal{M}_{\theta})^T v - \delta).
\end{equation}

Note, in the above equation, using multiple different values 
for $\delta$ provides us with the provision to effectively 
adjust and use a wide range of scores.
Then, we use a clip function to set the value greater 
than 0 in the score array, \emph{i.e.,} $(\text{scores}_{norm})$ to 0. 
Our salience map is based on this score, therefore, when the score is less than 0, it will appear in red, indicating that there is a potential wrong reasoning location.

An example of visualization is shown in 
Figure~\ref{fig:reading_case}, LLaMA-2-7B-chat did not really understand the meaning 
of the given question and misinterpreted 
``\emph{the distance covered by each train}'' as 
``\emph{the total distance covered by both trains}'', 
thus giving an incorrect reasoning path.
% Thus, all values less than 0 in scores are potential wrong reasoning positions.

\subsection{Representations Controlling}\label{sec:stage4}
\label{sec:RC}

Here we aim to correct the direction of the concept which may lead to CoT errors, as shown in the top right part of Figure \ref{fig:framework}. 

\liang{
Reviewer: "H[layer] ← H[layer] + v[layer]" what is the significance of this addition?
}

\liang{need to add linear representation and superposition hypothesis?}

\warn{
Given a query $x$, we adopt a simple process to control the direction of CoT. 
Specifically, as depicted in Algorithm~\ref{alg:control}, during the next token generation phase, we first acquire the reading vector $v$ from the concept identification phase.
Subsequently, we get the representations $H$ for the query $x$, and then we incorporate $v$ into the original representation weights of the corresponding control layers $L$ (as shown in line~\ref{line:addv} of Algorithm~\ref{alg:control}).
Finally, we transform the controlled representations $H$  into the logits of model for generation.
}


\eat{
\subsection{ Representations Controlling}\label{sec:stage4}
\label{sec:RC}
After the representations reading (section~\ref{sec:reading}), we aim to identify 
the direction and location of the concept which may where CoT goes wrong, as shown in the top right part of Figure \ref{fig:framework}. 
We adopt a simple process to control the direction of CoT.
Specifically, as shown in Algorithm~\ref{alg:control}, in the generation phase, we multiply the reading vector $v$ (obtained from section~\ref{sec:reading}) by a hyper-parameter $c$ and then add it to 
the original weight of the corresponding layers $L$. \di{Need more details}
}

% \input{tables/control_ag}

% representation_{raw}[layer] += coef * v

% where coeff is an adjustable coefficient parameter.
% \fixshu{Give its intuition + maths formulation}


% \subsection{Representation vs Prompt Engineering}
% \fixshu{Fill in details...!}
%%%%%%%%%%%%%%%%%% EXTRA TEXT %%%%%%%%%%%%%%%%%%%%%%%%%%


\eat{
Subsequently, the score is determined by calculating the dot product between the reading vector $v$ and representation 
$\text{Rep}(s_i, \mathcal{M}_\theta)$. 

We can represent the relevance between the stimulus representation and the latent concept based on this score.
}
\eat{
\eat{
\begin{equation}
    A_c = \text{mean}\{\text{Rep}(s_i, \mathcal{M}_\theta) \;|\; s_i \in T_{\text{LOC}_c} \}
\end{equation}
}
}
\eat{
\eat{
A natural choice in this regard is to select the subset of the representations (or collect neural activity) corresponding to the location of concept tokens $(c)$ in the prompt template $T_c$.
}
% \fixshu{why $T-C$ not introduced in Section~\ref{sec:select_stimuli}}
\eat{
For the cases with the target concept span multiple tokens,
}
}
\eat{
The sensitivity of large language models to different prompts 
is a crucial factor in the success of 
various carefully designed CoT mechanisms~\cite{sclar2023quantifying}. 

Since our work primarily focuses on the interpretability analysis of 
model CoT behavior in zero-shot and few-shot scenarios, it is 
essential to use different ``stimulus'' to \textit{induce} 
varying behaviors in the model. 

In Figure~\ref{fig:hopfieldianandstumili}, we illustrate 
how the concept of stimuli is transferred from cognitive 
neuroscience to large language models. In brief, when an LLM 
receives a positive stimulus $s^+$, it generates a specific 
output that, across a sample $x$, falls into the corresponding 
action space. Conversely, when it receives a negative 
stimulus $s^-$ or no stimulus at all, the model's output falls 
into a different action space $A^-$ or $A$. 


\warn{
Specifically, for zero-shot CoT, we append the text 
"\emph{Let's think step by step}" as a prompt 
prefix~\cite{kojima2022large}. 
This intends to explore how in zero-shot CoT 
this prompt prefix impacts the reasoning ability 
of LLMs.
For few-shot CoT, we use $n$ different example 
demonstrations~\cite{wei2022chain} prior to 
generating response from LLM.
For this, we aim to analyze, why providing 
examples can improve the reasoning accuracy of LLMs. 
An example illustration of pair of positive and 
negative prompt templates is given in 
Appendix~\ref{Appendix:Prompts_T} 
(Table~\ref{tab:prompt_for_stimulus}).
}

}



\eat{The core motivation of our work stems from the observations 
that discussed earlier confirm that CoT can improve the reasoning ability of LLM. However, few studies have conducted a comprehensive analysis of the interpretability of CoT. Inspired by work related to representation engineering~\cite{zou2023representation, Park2023linearhp}, the representations of LLM are almost secretly linear inside, and can be controlled via linear probe methods. These phenomena indicate that we can analyze the interpretability of CoT from the perspective of representation and control the thinking process of LLM.}



\eat{
The workflow of \OurMODEL{} is illustrated in Figure~\ref{fig:framework}
It encompasses the following different sub-components: 
(1) {Rationale Generation} (\S\ref{sec:BRG}), 
\eat{(2) Representation Reading (\S\ref{sec:RR}),} 
(2) Evaluation (\S\ref{sec:EV}) and 
(3) Control (\S\ref{sec:RC}). }

==> old_version/4b_experimental_setup.tex <==
\input{tables/zero_few_control}
\section{Experiments}
\subsection{Experimental Setup}
\noindent{\bf Dataset and Models.}
We consider 6 datasets for 3 different tasks: Arithmetic Reasoning, Commonsense Reasoning, and Symbolic Reasoning. For Arithmetic Reasoning, we select GSM8K~\cite{cobbe2021gsm8k} and SVAMP~\cite{patel-etal-2021-nlp}. Commonsense Reasoning is represented by StrategyQA~\cite{10.1162/tacl_a_00370} and CommonsenseQA (CSQA)\cite{talmor2019commonsenseqa}. Lastly, for Symbolic Reasoning, we include the Coin Flip\cite{wei2022chain} and Random Letter datasets, the latter constructed from the Last Letter dataset~\cite{wei2022chain}. More details and statistics of the datasets are provided in Appendix~\ref{Appendix:data} \syadd{We employ Llama-2-7B-chat~\cite{touvron2023llama} and Llama-3-8B-instruct~\cite{metallama3} to evaluate their precision performance (accuracy) both before and after applying control measures across the six datasets. Furthermore, we use the Llama-2-13B chat and the Llama-2-70B chat to ensure that our method performs effectively with larger-scale models.} 

\syadd{\noindent{\bf Three-Step Framework for Representation Control Experiments} \syinline{this title need to be rewrite}
For the Llama-2-7B-chat and Llama-3-8B-instruct models, we begin by using the original accuracy performance on the previously mentioned datasets as the baseline. Then we extract the zero-shot vector $v_z$ and few-shot vector $v_f$ using our proposed technique from the zero-shot and few-shot stimulus. This vector is then used to modify the models, resulting in the controlled models, denoted as $M_{zv^+}$. Next, we further enhance the zero-shot-augmented models by applying the few-shot vector, which produces the final models, denoted $M_{v_z^+v_f^+}$.} We evaluate $M_{zv^+}$ and $M_{v_z^+v_f^+}$ in previous dataset we mentioned. We use accuracy metrics for all dataset benchmarks. The answer extraction process is based on the methodology outlined by~\citet{kojima2022large}. Detailed procedures and results are provided in the Appendix~\ref{Appendix:extract}.


\syinline{need to be clear and add a illustrate figure or demo} 


In order to extract the vectors, we explore the number of samples $n$ in stimulus, see more details in our ablation study section~\ref{section:ablation study}.

We pick the last five layers to control the reasoning direction\syinline{you shoule definiation what is the reasoning direction first} of the LLM and select 128 stimulus samples according to our abulation experiment. Specifically,  
For experimentation, we use a value of threshold $\delta$ = 3.5.
 
coeff=1.8
We use float16 to load large models. We employ greedy search as our decoding strategy and set max new tokens of 512 for all datasets. All experiments are conducted 
using NVIDIA L20 GPU.



\syadd{
\subsection{Ablation Experiments}
\label{section:ablation study}
\syadd{\noindent Explore the optimal number of samples to be a stimulu}

$n_{train}$

We conducted experiments using three distinct reading set sizes:,32,64,128,256 and 512 amples, details shown in Appendix~\ref{Appendix:reading_size}.

\syadd{\noindent Explore the layers for LLM reasoning control}
The abstract feature will located in which layers? 

layer 2-6
last 5 layers 
last 10 layers 
last 15 layers 

\syadd{\noindent The selection method of the samples}

hard question 

ppl 

ppl + hard questions

}

what about the coeff=1.8?




\noindent{\bf Implementation Details.}



In our study, we pick the last ten layers to control the reasoning direction of the LLM and select different numbers of stimulus samples according to different tasks. Specifically, We conducted experiments using three distinct reading set sizes: 128, 256, and 512 samples, details shown in Appendix~\ref{Appendix:reading_size}. 
For experimentation, we use a value of threshold $\delta$ = 3.5.
We use float16 to load large models. We employ greedy search as our decoding strategy and set max new tokens of 512 for all datasets. All experiments are conducted 
using NVIDIA L20 GPU.

\eat{
In our study, we select different numbers of stimulus samples according to different tasks. Specifically, 
% \warn{This line does not match with the bullets given below...?}
}
% \begin{itemize}
% \itemsep0em 
%     \item coeff - We incorporate the explained variance ratio from the principal components into the control process to stabilize and standardize the coeff values across various model configurations, thereby enhancing the adaptability of control process.
%     \item layers - The specific layers utilized in our experiments are meticulously selected based on their model performances.
%     \item number of train datasets in reading representation - We conducted experiments using three distinct reading set sizes: 128, 256, and 512 samples.
%     \item answer extraction - The answer extraction process is based on the methodology outlined by~\citet{kojima2022large}. Detailed procedures and results are provided in the Appendix~\ref{Appendix:extract}.
% \end{itemize}
% \warn{ What are these parameters ``coeff'', ``layers''..?\\
% they are not introduced before..!}



\eat{
\noindent{\bf Experimental Settings.}
For experimentation, we use value of threshold $\delta$ = 2.
We use float16 to load large models. We employ greedy 
search as our decoding strategy, and set max new tokens 
of 512 for all datasets. All experiments are conducted 
using NVIDIA L20 GPU.
}



% \subsection{CoT error Definition}
% Based on the experimental results, we classify the errors generated by CoT into the following categories: 
% \fixshu{Also Give short names to these error categories.}

% \begin{enumerate}
% \itemsep0em 
%     \item \warn{X} Method is wrong. It denotes an error in the method of thinking during the chain of thought, where the overall thought deviates from the correct path of disintegration, from to embodied in a holistic error.
%     \item \warn{Y} Method correct but process wrong. It indicates that the holistic problem solving idea is correct, but there is a partial error in the process of it, which leads to a question answering error, a localized error.
%     \item \warn{Z} Prediction correct but process wrong. This is a case where the prediction turned out to be correct, but the thought process was wrong. The model coincidentally predicted the correct answer.
% \end{enumerate}


\eat{
\subsection{Top down Interpretability Analysis of CoT with Representation }
\warn{This section we must need?}
\paragraph{Representation Read}
\paragraph{Representation Control}
}


==> old_version/7b_limitation.tex <==
\section*{Limitations}
Our current problem formulation is primarily focused
on text data. We consider multi-modal scenarios, \emph{i.e.,} analyzing concepts from multiple different modalities as a future research direction.

%\section*{Ethics Statement}
%Our framework can provide intuitive and interpretable analysis for CoT reasoning, which is helpful in tracing and controlling the errors LLMs made during the CoT process. This poses an impact on rectifying LLMs' reasoning paths and enhancing CoT's transparency. 

\eat{
Some of the limitations of our work are as follows:
\warn{1. Limited number of base models: The number of base models used was inadequate, preventing a thorough evaluation of model performance. 2. Lack of comparison across different shots: The study did not compare the performance of models under varying shots conditions, which restricts the comprehensiveness of the results.}
\warn{Fill details. Limitation is mandatory in ACL submissions.}
}
% \begin{enumerate}
% \itemsep0em    
%     \item 
% \end{enumerate}


==> section/4_method.tex <==
\section{Bridging Reasoning in CoTs and the Hopfieldian View}
\label{sec:method}
In this section, we aim to build a bridge between the reasoning process in CoTs and the Hopfieldian view of cognition. We will particularly associate the main elements with the Hopfieldian view.  After understanding these elements, we can leverage the strength of the Hopfieldian view to improve the current CoTs. Note that for other elements, such as attractors, state space, and basin of attraction, we will leave it as future work. 

\noindent {\bf Stimuli and Actions.} Stimuli and action are key components of how the brain processes information and interacts with the environment. Action refers to the motor responses or behaviors that result from cognitive processing, which is the response given by LLMs via CoTs. Stimuli refer to external or internal events, objects, or changes in the environment that are detected by the sensory systems and can influence cognitive processes and behavior. In CoTs, it corresponds to the specific text in its prompts. For the zero-shot setting, we define the stimuli as $s_{zero}$ to represent a set of supplementary instructions in the prompt that encourage the model to provide more intermediate reasoning steps before arriving at a final answer. For example, it can be ``\textit{let's think step by step}'' and ``\textit{make sure to give steps before your answer}''. In the few-shot setting, the stimuli $s_{few}$ is defined as a sequence of demonstrations $Q=\{(\tilde{q}_1, \tilde{a}_1), (\tilde{q}_2, \tilde{a}_2), \dots\}$, where $\tilde{q}_i$ represents the query and $\tilde{a}_i$ is the corresponding response. In the following discussion, we use $s^+$ to indicate that stimuli are included in the model's input and $s^-$ to indicate that no stimuli are added. We avoid using explicitly negative stimuli, such as ``\textit{please be careless and answer the following question}'', because a well-aligned model would likely refuse to behave in such a manner~\citep{ouyang2022training}.

\noindent {\bf Neural Populations.} As we mentioned, in the Hopfieldian view, representations can be realized by various forms of neural organization, especially populations. Identifying these neural populations in CoTs is especially important. In our framework, there are two steps. 

(i) Stimuli Set Design. Firstly, our goal is to elucidate the sensitivity of LLMs to different CoT prompts with stimuli. In detail, we construct a prompt dataset. For each query $q$, there are two forms of prompts: positive one (with stimuli) as $p^+ = p(s^+, q)$ and negative one (without stimuli) as $p^- = p(s^-, q)$, where $p$ is the prompt template. Specifically, for each query $q_i$, we construct $M$ number of prompts for both of them with different stimuli, which is denoted as $P_{i} = \{p_1^{i,-}, p_1^{i,+}, p_2^{i,-}, p_2^{i,+}, \dots, p_M^{i,-}, p_M^{i,+}\}$. Thus, in total, we have a stimuli set $P^{*} = \{P_1, P_2, \cdots, P_{N} \}$. When an LLM receives a prompt $p^+$ containing a positive stimulus $s^+$, it generates a specific response $a^+$, which falls within the corresponding action space $A^+$. Conversely, when the model receives a negative stimulus $p^-$, its output falls into a different action space $A^-$. These contrastive pairs of prompts will be used to identify neural populations given by these stimuli. 

(ii) Identifying Neural Populations. Generally, the neural populations should be the most influential activation vectors given by these prompts or stimuli. In detail, for each prompt in the $P^*$, the next step is capturing the network architecture's corresponding neural populations. Since LLMs rely on transformer-based architecture to store distinct representations intended for different purposes, it is crucial to design the extraction process to capture task-specific representations carefully. For a given prompt $p^+$ or $p^-$, we need to find the `most representative token', which encapsulates rich and highly generalizable representations of the stimuli. 
Here we select the \emph{last token}, which is based on the observation in \citep{zou2023representation} that it is the most informative token
for decoder-only or auto-regressive architecture models. 

Once the last token position is identified, we can naturally select some of its activations in hidden layers as its neural populations. Previous studies have shown that not all layers store important information; here, we focus on a subset of them to reduce the computation cost, whose indices are denoted as a set $\mathcal{K}$ (in practice, $\mathcal{K}$ is always the last several layers). Thus, we have a collection of activation vectors, i.e., neural populations for the prompt, given by these layers $H_{\mathcal{K}}(p)=\{h_k(p)\}_{k\in \mathcal{K}}$, where $h_k(p)$ refers to the activation vector of the $k$-th layer for a given input prompt $p$. 

Based on this, for each hidden layer in $\mathcal{K}$, we have the neural population for all prompts, which is denoted as 
\begin{equation}\label{eq:neural}
h^{*}_k = \{ h_k(P_1), h_k(P_2), \ldots, h_k(P_N) \}.
\end{equation}

\noindent {\bf Representation Spaces.}  
After we have the neural populations for each selected hidden layers. Our final goal is to find the representation space. In the Hopfieldian view, the representation of information is thought to occur within low-dimensional space embedded within higher-dimensional neural spaces. Thus, these representation spaces will be the most informative subspaces of the neural populations. Here we adopt the PCA to find such a $k$ dimensional subspace. Specifically, for the $k$-th layer where $k\in \mathcal{K}$, we perform PCA analysis on $h_k^*$ in (\ref{eq:neural}): \lladd{the input of PCA is a set of difference? $h_k^*$ is the set of activation vector.}
\begin{equation}\label{eq:2}
    R_k=\text{PCA}(h_k^*). 
\end{equation}
Then, the space spanned by this eigenvector will be the representation space for this layer.  

\section{Applications of Hopfieldian View to CoTs} 
In the previous section, we mainly discussed how each element in the Hopfieldian view corresponds to the reasoning in CoTs. From our previous view, we can understand the reasoning process as the movement between these representation spaces. Based on these connections, we can, in fact, leverage the strength of the Hopfieldian view to improve or further understand CoTs. In this section, we first consider how to localize the reasoning error based on the low dimensional representation spaces. Then, by leveraging the robustness of the Hopfieldian view, we propose a new framework, namely Representation of Thought, that enhances the performance robustness of CoTs. 

\subsection{Reasoning Error Localization}
As in the Hopfieldian view, cognition occurs within low-dimensional representation spaces. Reasoning errors can be identified by analyzing the structure of these spaces, such as when certain dimensions (representing specific cognitive factors) are disproportionately activated or suppressed. This can help localize the source of the error within the cognitive process. Motivated by this, we can leverage the internal structure of spaces we have learned via PCA to locate the reasoning error for a given query in CoTs.

Intuitively, for a given query, to localize whether it has reasoning errors, we can check whether its neural populations are close to the corresponding representation spaces we learned in the previous section. This is because the reasoning occurs within these representation spaces, if neural populations are far from the spaces, that means CoTs cannot understand the corresponding concepts. Mathematically, given a query $x$, we format it using the stimulus prompting template and represent it as $p$. By using a similar procedure as in Neural Populations in the previous section, we can get its neural populations $\{h_k(p)\}_{k\in \mathcal{K}}$.  Then we use the following criterion to access and/or evaluate the quality of the rationales at the $k$-th layer:
\begin{equation}
    \text{scores}_k(p) =  h_k(p)^\top R_k - \delta, 
\end{equation}
$R_k$ is the principal eigenvector we get for the $k$-th layer in the previous section. 
Note that in the above equation, using multiple different values 
for $\delta$ provides us with the provision to effectively 
adjust and use a wide range of scores.
When the score is less than 0, it indicates that there is a potential wrong reasoning location.

\subsection{Representation of Thought} 
The Hopfieldian view of cognition offers a framework that can potentially be used to control or influence cognitive processes.  Specifically, influencing neural populations directly offers a more robust way to control cognition compared to simply providing different stimuli. Firstly, influencing neural populations directly allows the manipulation of the core dynamics of neural state spaces, including attractor states, bifurcations, and transitions between cognitive states. This direct intervention bypasses the variability and unpredictability associated with external stimuli, which depend on the individual’s perception, attention, and prior experiences. Moreover, external stimuli are subject to various forms of noise and variability, including sensory processing errors, environmental distractions, and individual differences in interpretation. Direct manipulation of neural populations can reduce these sources of noise, providing a cleaner and more consistent pathway to controlling cognitive states.

Our RoT leverages representation spaces' structure to enhance the robustness of reasoning in CoTs. Intuitively, we can manipulate a given query's neural populations to be closer to these representation spaces to enhance robustness since they are the inherent entities in the reasoning process. After the manipulation, the neural populations (hidden states) will be less dependent on the specific form of the prompt, query, and stimuli. Mathematically, given a query $x$, we format it using the stimulus prompting template and represent it as $p$.  By using a similar procedure as in Neural Populations in the previous section, we can get its neural populations $\{h_k(p)\}_{k\in \mathcal{K}}$. In RoT, we will manipulate them by injecting a vector in their corresponding representation spaces to make them closer to these spaces. 
\begin{equation}
    h'_k(p) = \begin{cases} 
        h_k(p) + \alpha R_k & \text{if } k \in \mathcal{K} \\
      h_k(p) & \text{otherwise}
          \end{cases}
\end{equation}
where  $h'_k(p)$ denotes the manipulated hidden state, $\alpha$ is a scaling factor controlling the manipulation strength. Its sign should follow the sign of $ h_k(p)^\top R_k$. 

By directly manipulating neural populations, RoT offers a more precise and interpretable method for influencing the model's output compared to traditional prompt engineering techniques. This approach not only enhances control over the model's behavior but also improves the transparency and predictability of the generation process.



















%%%%%%%%%%%%%%%   Extra Stuff   %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Specifically, we implement the impact of stimulus in Hopfieldian view as follows: we define a set of positive stimulus $S^{+} = \{s^{+}_i \mid i = 1, \dots, M\}$ and corresponding negative stimulus $S^{-} = \{s^{-}_i \mid i = 1, \dots, M\}$, where $M$ denotes the number of stimuli. This allows us to generate a set of prompts $P_{i} = \{p_1^{i,-}, p_1^{i,+}, p_2^{i,-}, p_2^{i,+}, \dots, p_M^{i,-}, p_M^{i,+}\}$ for sample $i$, where $p_m^{+}$ represents the $m$-th positive stimuli and $p_m^{-}$ represents the $m$-th negative stimuli, respectively. Then, for the $N$ test samples we choose to stimuli, we have the prompt set $P^{*}$ with stimulus set $S^{+}$ and $S^{-}$, \ie $P^{*} = \{P_1, P_2, \cdots, P_{N} \}$. When an LLM receives a prompt $p^+$ containing a positive stimulus $s^+$, it generates a specific response $a^+$ to the query $q$, which falls within the corresponding action space $A^+$. Conversely, when the model receives a negative stimulus $p^-$, its output falls into a different action space $A^-$.

%Let $h_l, l\in [M]$ represent the $l$-th layer's hidden state of LLM with $L$ layers.
%The index subset of selected hidden layers can be denoted as $\mathcal{K}$, in which $K$ is the total number of our selected layers. %
%Note that $k \in \mathcal{K}$ represents the index of selected layers. 
%For example, the subset can be $\{ h_2, h_4, h_6, h_8, h_{10} \} $ corresponds to $\mathcal{K} = \{ 1,2,3,4,5 \}$. Then the activations of these layers are represented as:

\iffalse 
Next, we extract a set of hidden states, denoted as:
\begin{equation*}
H_{\mathcal{K}}(p) =  \{h_k(p) \}_{k \in \mathcal{K}}.
\end{equation*}
We collect the activations of the hidden states from the prompts set $P^{*}$, which we construct based on a set of stimuli from the previous step.
For each selected layer index $k$, the activations triggered by the $M$ stimuli across $N$ samples are denoted as $h^{*}_k$, and are defined as:
\begin{equation*}
h^{*}_k = \{ h_k(P_1), h_k(P_2), \ldots, h_k(P_N) \},
\end{equation*}
where $P_1, P_2, \ldots, P_N$ are the prompts for $M$ positive and negative stimuli across $N$ test samples. And the $h^{*}_k$ is our \emph{neural population} in the Hopfieldian view.

Then, for the total $K$ selected layers, the neural activations collection is denoted as $H^{*}_\mathcal{K}$, which is defined as:
\begin{equation}
H^{*}_\mathcal{K} = \{ h^{*}_1, h^{*}_2, \ldots h^{*}_K\},
\end{equation}
where $H^{*}_\mathcal{K}$ encompasses the activations from all selected layers in the index subset $\mathcal{K}$, triggered by the set of stimulus $P^{*}$.
\fi 

\iffalse 
In the previous step, we derived the activations triggered by the $M$ stimuli across $N$ samples for the layer index $k$, \ie $h^{*}_k$. Then, for each selected layer, we use Principal Components Analysis (PCA) to find the $u$ representative vectors denoted as $R$, which constitutes the \emph{neural space} in each selected layer. Specifically, let $h_k^i$ denotes the $i$-th element of the vector $h^{*}_k$, $\tilde{h}_k = h^{*}_k - \mu_k$ denote the centered hidden states, where $\mu_k = \frac{1}{2MN}\sum_{i=1}^{2MN} h_k^i$. Then, we find the representations in the $k$-th layer as: 
\begin{equation}
R_k = \argmax_{U} \text{tr}((U)^T \tilde{h}_k (\tilde{h}_k)^T U), 
\end{equation}
subject to $U^T U = \mathbb{I}$. Where tr is the trace of the matrix, and $U$ is our representation vectors, \ie each column is a representation vector. The span of the representation vectors is our representation space or \emph{neural space}. $\text{Span}(R_k)$. 
\fi 

\eat{For each $R_k$, we determine its sign $sign_k \in \{-1, 1\}$ by:
\begin{equation*}
sign_k = sign \left( \frac{1}{NM} \sum_{i=1}^{NM} [\argmax_{j \in \{0,1\}} (h_k(p_i^j))^T R_k] - \frac{1}{MN} \sum_{i=1}^{NM} [\argmin_{j \in \{0,1\}} (h_k(p_i^j))^T R_k] \right),
\end{equation*}
where $N$ is the number of sample, $M$ is the number of stimuli, $j$ denotes the stimuli associated with the prompt, $j=1$ indicates that the prompt has a positive stimulus $s^+$. If $sign_k$ is positive, it indicates that the positive stimulus $S^+$ is more aligned $R_k$ compared to the negative stimulus. In other words, from a Hopfield view, this means that the direction of the representation vector is more aligned with moving from negative action space $A^-$ towards positive activation space $A^+$. Then, the adjusted representation of thought $R_s$ for reasoning stimuli $P^{*}$ can be given by $R_k \times sign_k$.}

\iffalse 
In this section, we will dive into details about our motivation from the  Hopfieldian view and a general introduction to our framework. 

\noindent{\bf Motivation.} Existing literature has confirmed that CoT can improve the reasoning ability of LLMs~\citep{kojima2022large,wei2022chain}. 
However, few studies have conducted a comprehensive analysis of the interpretability of CoT. This is mainly because reasoning is a complex task, and the model's final performance is influenced by numerous factors. \llinline{do we need to add some cites here?} 
Analyzing internal activations in isolation or from the perspective of individual neurons of LLMs is challenging. Inspired by work related to representation engineering~\citep{zou2023representation}, we consider LLM from a higher-level cognition perspective (Hopfieldian view), \ie specific external stimuli activate representations within the model, thereby causing the model to exhibit different behaviors that represent the population activation behavior of neurons within the model. Meanwhile, many studies have shown that the representations of LLM are almost secretly linear inside, and can be controlled via linear probe methods~\citep{Park2023linearhp,wu2024reft}.
These phenomena indicate that we can analyze the interpretability of CoT from the perspective of representation and control the reasoning process of LLM.

\input{tables/fig1}

\di{This should be your motivation}
Building on this line of work, we propose Representations of Thought, which first extracts interpretable representations of zero-shot and few-shot reasoning, and then uses these representations to control the model's behavior, as illustrated in Figure~\ref{fig:rotframework}.

\input{tables/framework_example}
When a large language model $M_\theta$ processes a prompt containing zero-shot instructions $P(I,q)$ or few-shot demonstrations $P(D,q)$, what representations emerge, and how do these representations facilitate reasoning? \di{make your notations consistent!} To explore this question, we present our RoT framework based on the Hopfieldian view.  \di{Now I know representing and CoT, but I still cannot get the relation between Hopfieldian view of our framework! I think you need to mention the relation between Hopfieldian view and representation, right? }
Hopfieldian demonstrates that each prompt $P$ contains a set of stimuli $S$, which can trigger distinct neural activations in LLMs, leading to specific actions $A$. While it's impossible to determine the activation of each individual neuron in large-scale models, we can identify representations $R$ based on patterns of activity across neuronal populations, drawing on the research of~\citet{barack2021twoviews}. Our framework can be divided into two components: (1) Extract the representations of thought (2) Control LLMs' reasoning behavior with RoT. An illustrated example of our framework is provided in Figure~\cite{fig:rotframework_hidden}

\noindent{\bf Framework.}
As we are targeting at exploiting the Hopfieldian view to provide an explanation for LLMs' CoT reasoning, we have to build a bridge from the components in the cognitive brain to CoTs. We begin from introducing the definition of stimulus in CoT, which is the prompt text (\ie example input-output demonstrations in a few-shot scenario and \emph{``think step by step''} in a zero-shot scenario). Then use these stimuli to activate specific "neural populations" for CoT.

For neural populations, ideally, we can leverage humanly comprehensible concepts within LLMs' representations. To model these concepts, our framework has two phases: 
(i) \emph{Concept Modeling},  and (ii) \emph{Concept Simulation}. 
In the Concept Modeling phase (Section \ref{sec:stage1}), LLMs will learn latent (both concrete and abstract) concepts from pertaining documents, and these concepts might pertain to specific names or domains, such as ``medical'' or ``climate change''. 
They could also represent more abstract notions derived from document-level modeling, such as ``positive language'', ``careful reasoning'', or ``affirmative expression''. 
Likewise, in the Concept Simulation stage (Section \ref{sec:stage2}), zero-shot or few-shot prompts serve as stimuli for the LLM, inducing the activation of specific concepts. 
These activated concepts collectively determine the final action of this model.

However, directly extracting activated concepts would consume a tremendous amount of computational resources, and individual concepts alone cannot determine the model's overall action. 
Therefore, our framework uses representations to denote the activation of concepts when the model is stimulated. 
For this, our framework employs \emph{Representations  Reading} (Section \ref{sec:stage3}) and \emph{Representations Controlling} (Section \ref{sec:stage4}) as the core modeling components.  

Next, we will give details about the individual model components. Later, we explain how this framework can be used to improve the CoT reasoning abilities of LLMs. See Figure \ref{fig:framework} for an illustration of our framework.  

\subsection{Framework of RoT}
\di{What is the goal of this step?} The whole extraction pipeline can be broken down into three steps: i) Design zero-shot and few-shot \textit{stimulus}. ii) Collect \textit{neural activations}. iii) Extract \textit{representation vectors} from activations. 

\textbf{(i) Stimuli Design.} Firstly, to elucidate the sensitivity of LLMs to different CoT prompts with signal strength, in this step, we will employ "\emph{stimuli}" inducing diverse model behaviors under both zero-shot and few-shot settings. Our objective is to analyze how the prompts corresponding to a specific stimulus are processed and transferred within large models, as illustrated in Figure~\ref{fig:hopfieldianandstumili}, from the perspective of cognitive neuroscience. For the zero-shot setting, we define the stimuli as $s_{zero}$ to represent a set of supplementary instructions in the prompt that encourage the model to provide more intermediate reasoning steps before arriving at a final answer, for example, it can be "let's think step by step" and "make sure to give steps before your answer". In the few-shot setting, the stimuli are defined as $s_{few}$, a sequence of demonstrations $(q_1, a_1), (q_2, a_2), \dots, (q_i, a_i),\dots$, where $q_i$ represents the query and $a_i$ is the corresponding response. In the following discussion, we use $s^+$ to indicate that stimuli are included in the model's input, and $s^-$ to indicate that no stimuli are added. We avoid using explicitly negative stimuli, such as "please be careless and answer the following question," because a well-aligned model would likely refuse to behave in such a manner~\citep{ouyang2022training}.

Next, we construct a dataset of contrasting prompt pairs. In each pair, the prompt $p$ is presented in two forms: positive (with stimuli) as $p^+ = p(s^+, q)$ and negative (without stimuli) as $p^- = p(s^-, q)$, where $q$ represents the original query. Specifically, we implement the impact of stimulus in Hopfieldian view as follows: we define a set of positive stimulus $S^{+} = \{s^{+}_i \mid i = 1, \dots, M\}$ and corresponding negative stimulus $S^{-} = \{s^{-}_i \mid i = 1, \dots, M\}$, where $M$ denotes the number of stimuli. This allows us to generate a set of prompts $P_{i} = \{p_1^{-}, p_1^{+}, p_2^{-}, p_2^{+}, \dots, p_M^{-}, p_M^{+}\}$ for each test sample $i$, where $p_m^{+}$ represents the $m$-th positive stimuli and $p_m^{-}$ represents the $m$-th negative stimuli, respectively. Then, for the $N$ test samples we choose to stimuli, we have the prompt set $P^{*}$ with stimulus set $S^{+}$ and $S^{-}$, \ie $P^{*} = \{P_1, P_2, \cdots, P_{N} \}$. When an LLM receives a prompt $p^+$ containing a positive stimulus $s^+$, it generates a specific response $a^+$ to the query $q$, which falls within the corresponding action space $A^+$. Conversely, when the model receives a negative stimulus $p^-$, its output falls into a different action space $A^-$.



\textbf{(ii) Neural Activations Collection.} After receiving the task-specific prompt stimuli, the next step is to capture the corresponding representations from the LLM. For a given input prompt $p^+$ or $p^-$, we retrieve the hidden state values at the index of the `most representative token', which encapsulates rich and highly generalizable representations of the stimuli or task. Since LLMs rely on transformer-based architecture to store distinct representations intended for different purposes, it is crucial to design the extraction process to capture task-specific representations carefully. 

For decoder-only or auto-regressive architecture models, one natural choice is to select the position of the \emph{last token} as the  `most representative token'~\citep{radford2018improving,zou2023representation}. Once the suitable token position is identified, we then select a subset of hidden layers to extract their activations, see Appendix~\ref{app:parameter} for our exploration of layer selection. Let $h_l$ represent the $l$-th layer's hidden state of LLM, with the hidden layers indexed from 1 to $L$, where $L$ is the total number of the LLM layers. The subset index of selected hidden layers can be denoted as $\mathcal{K} = \{ 1,2,..., K \}$, in which $K$ is the total number of our selected layers. Note that $k \in \mathcal{K}$ represents the index of selected layers. For example, the subset can be $\{ h_2, h_4, h_6, h_8, h_{10} \} $ corresponds to $\mathcal{K} = \{ 1,2,3,4,5 \}$. Then the activations of these layers are represented as:
\begin{equation*}
\{h_k(p) | k \in \mathcal{K}\},
\end{equation*}
where $h_k(p)$ refers to the activations of layer index $k$ for a given input prompt $p$, and $\mathcal{K}$ contains the indices of the hidden layers we select for activation. Next, we extract a set of hidden states, denoted as:
\begin{equation*}
H_{\mathcal{K}} =  \{h_k(p) \}_{k \in \mathcal{K}}.
\end{equation*}
We collect the activations of the hidden states from the prompts set $P^{*}$, which we construct based on a set of stimuli from the previous step.
For each selected layer index $k$, the activations triggered by the $M$ stimuli across $N$ samples are denoted as $h^{*}_k$, and are defined as:
\begin{equation*}
h^{*}_k = \{ h_k(P_1), h_k(P_2), \ldots, h_k(P_N) \},
\end{equation*}
where $P_1, P_2, \ldots, P_N$ are the prompts for $M$ positive and negative stimuli across $N$ test samples. And the $h^{*}_k$ is our \emph{neural population} in the Hopfieldian view.

Then, for the total $K$ selected layers, the neural activations collection is denoted as $H^{*}_\mathcal{K}$, which is defined as:
\begin{equation}
H^{*}_\mathcal{K} = \{ h^{*}_1, h^{*}_2, \ldots h^{*}_K\},
\end{equation}
where $H^{*}_\mathcal{K}$ encompasses the activations from all selected layers in the index subset $\mathcal{K}$, triggered by the set of stimulus $P^{*}$.

\textbf{(iii) Extract Representative Vectors.} 
In the previous step, we derived the activations triggered by the $M$ stimuli across $N$ samples for the layer index $k$, \ie $h^{*}_k$. Then, for each selected layer, we use Principal Components Analysis (PCA) to find the $u$ representative vectors denoted as $R$, which constitutes the \emph{neural space} in each selected layer. Specifically, let $h_k^i$ denotes the $i$-th element of the vector $h^{*}_k$, $\tilde{h}_k = h^{*}_k - \mu_k$ denote the centered hidden states, where $\mu_k = \frac{1}{2MN}\sum_{i=1}^{2MN} h_k^i$. Then, we find the representations in the $k$-th layer as: 
\begin{equation}
R_k = \argmax_{U} \text{tr}((U)^T \tilde{h}_k (\tilde{h}_k)^T U), 
\end{equation}
subject to $U^T U = \mathbb{I}$. Where tr is the trace of the matrix, and $U$ is our representation vectors, \ie each column is a representation vector. The span of the representation vectors is our representation space or \emph{neural space}. 

For each $R_k$, we determine its sign $sign_k \in \{-1, 1\}$ by:
\begin{equation*}
sign_k = sign \left( \frac{1}{NM} \sum_{i=1}^{NM} [\argmax_{j \in \{0,1\}} (h_k(p_i^j))^T R_k] - \frac{1}{MN} \sum_{i=1}^{NM} [\argmin_{j \in \{0,1\}} (h_k(p_i^j))^T R_k] \right),
\end{equation*}
where $N$ is the number of sample, $M$ is the number of stimuli, $j$ denotes the stimuli associated with the prompt, $j=1$ indicates that the prompt has a positive stimulus $s^+$. If $sign_k$ is positive, it indicates that the positive stimulus $S^+$ is more aligned $R_k$ compared to the negative stimulus. In other words, from a Hopfield view, this means that the direction of the representation vector is more aligned with moving from negative action space $A^-$ towards positive activation space $A^+$. Then, the adjusted representation of thought $R_s$ for reasoning stimuli $P^{*}$ can be given by $R_k \times sign_k$.

\subsection{Control Reasoning Behavior with RoT} After extracting the representation for a specific stimulus, RoT enables fine-grained control over the model's generation process without requiring full fine-tuning or extensive prompt engineering. This representation is selectively injected into predetermined layers of the model during the forward pass:
\begin{equation}
    h'^{(l)} = \begin{cases} 
        h^{(l)} + \alpha r_s & \text{if } l \in L \\
        h^{(l)} & \text{otherwise}
    \end{cases}
\end{equation}
where $h'^{(l)}$ denotes the injected hidden state, $h^{(l)}$ represents the original hidden state, $\alpha$ is a scaling factor controlling the injection strength, and $L_s$ is the set of layers selected for injection.
By directly manipulating hidden states, RoT offers a more precise and interpretable method for influencing the model's output compared to traditional prompt engineering techniques. This approach not only enhances control over the model's behavior but also improves the transparency and predictability of the generation process.


\fi 


==> tables/LAT_algo.tex <==
\begin{algorithm}[t]
    \caption{LAT Process-flow}
    \label{alg:LAT}
    \KwIn{Stimulus set $S$, model $\mathcal{M}_{\theta}$, function $Rep(.,.)$}
    \KwOut{Reading vector $v$}

    $A_c \gets []$ \tcp{neural activity list}
    
    \For{$s_i$ \textbf{in} $S$}{
        $A_c \gets A_c + [Rep(s_i, \mathcal{M}_{\theta})[-1]]$ 
    }
    
    $i \gets 0$
    
    $D \gets []$ \tcp{difference list}
    
    \While{$i < len(S) - 1$}{
        $D \gets D + [A_c[i+1] - A_c[i]]$ \label{line:diff}

        $i \gets i + 2$
    }

    $v \gets \text{PCA}(D)[0]$

    \textbf{return} $v$
\end{algorithm}

% \begin{algorithm}
% \caption{The process of MMAD}
% \label{alg:framework}
% % \SetAlgoLined
% \KwIn{Debate topic $t$, maximum number of rounds $N$, text debater $\mathcal{T}$, multi-modal debater $\mathcal{M}$ and judge debater $\mathcal{J}$}
% \KwOut{Final answer $a$}

% \emph{Initialize the opinions for all debaters}

% $O_t \leftarrow \mathcal{T}(text)$

% $O_m \leftarrow \mathcal{M}(text, image)$

% $D \leftarrow [\mathcal{T}, \mathcal{M}]$

% $H \leftarrow [t, O_t, O_m]$

% $n \leftarrow 0$ 

% \While{$n \le N$}{
%     $n \leftarrow n + 1$

%     \For{each $D_i \in D$}{
%         $h \leftarrow D_i(H)$

%         $H \leftarrow H + [h]$
%     }
%     \If{$J_d(H)$}{break}

% }

% $a \leftarrow J_e(H)$
% \end{algorithm}


==> tables/RoT_framework.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]
    {figures/RoT_framework.pdf}
    \caption{An overview of Presentation of Thought (RoT)}
    \label{fig:rotframework}
\vspace{-20pt}
\end{figure*}


==> tables/ablation_N_L.tex <==
\begin{figure*}[t]
\centering
\begin{minipage}[t]{0.40\textwidth}
  \centering
  \includegraphics[width=\textwidth]{figures/ntrain.pdf} 
  \subcaption{Results for different numbers of samples in the stimulus set.}
  \label{subfig:ntrain}
\end{minipage}
\hfill
\begin{minipage}[t]{0.40\textwidth}
  \centering
  \includegraphics[width=\textwidth]{figures/layer.pdf}
  \subcaption{Results for different numbers of last layers for neural populations.}
  \label{subfig:layer}
\end{minipage}
\caption{Ablation study of our approch on the SVAMP dataset.}
\label{fig:ablation_parameter}
\vspace{-12pt}
\end{figure*}


==> tables/app_few_shot.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/app_few_shot.pdf}
    \caption{A example of using Few-shot CoT.}
    \label{fig:app_few_shot}
\vspace{-7pt}
\end{figure}

==> tables/app_zero_shot.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/app_zero_shot.pdf}
    \caption{A example of using Zero-shot CoT.}
    \label{fig:app_zero_shot}
\vspace{-7pt}
\end{figure}








==> tables/arithmetic_reasoning_result_table.tex <==
\begin{table*}[ht]
\centering
% \small
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{lcccc}
\hline
\multirow{2}{*}{Model} & \multicolumn{3}{c}{Arithmetic Reasoning} \\ \cline{2-4} 
 & GSM8K & SVAMP & AQuA \\ \hline
\multicolumn{4}{c}{zero-shot CoT} \\ \hline
Mistral-7B-instruct & 45.03 / \textbf{47.08} & 57.33 / \textbf{61.33} & 25.59 / \textbf{30.71} \\
LLaMA-2-7B-chat & 26.31 / \textbf{27.37} & 46.00 / \textbf{46.67} & 27.95 / \textbf{30.71} \\
LLaMA-3-8B-instruct & 74.45 / \textbf{75.89} & 82.67 / \textbf{84.00} & 42.13 / \textbf{45.67} \\ 
Avg. & 48.60 / 50.11 (\textbf{1.51↑}) & 62.00 / 64.00 (\textbf{2.00↑}) & 31.89 / 35.70 (\textbf{3.81↑})  \\ \hline
\multicolumn{4}{c}{few-shot CoT} \\ \hline
Mistral-7B-instruct & 46.78 / \textbf{47.16} & 61.33 / \textbf{61.67} & 34.65 / \textbf{35.04} \\
LLaMA-2-7B-chat & 5.00 / \textbf{5.16} & 38.67 / \textbf{39.00} & 22.44 / \textbf{23.62} \\
LLaMA-3-8B-instruct & 72.71 / \textbf{74.83} & 82.00 / \textbf{83.67} & 52.76 / \textbf{53.21} \\
Avg. & 41.50 / 42.38 (\textbf{0.88↑}) &  60.67 / 61.45 (\textbf{0.78↑}) & 36.61 / 37.29 (\textbf{0.68↑}) \\ \hline
\end{tabular}
}
\caption{Results on the Arithmetic Reasoning task for different models. The left side shows scores without control, and the right side shows scores after control.}
\label{tab:arithmetic_result}
\vspace{-7pt}
\end{table*}

==> tables/case_aqua_zero.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/case_aqua_zero.pdf}
    \caption{A real case predicted by LLaMA-3-8B-instruct with zero-shot CoT on the AQuA dataset. 
    The segment highlighted in \textcolor{skyblue}{blue} represents the correct output of the model. 
    The \textcolor{crimson}{red} part shows that the model starts to reason in the wrong direction without control, 
    while the \textcolor{seagreen}{green} portion indicates the model reason in the correct direction after adding control.}
    \label{fig:case_aqua_zero}
\end{figure*}








==> tables/case_coin_few.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/case_coin_few.pdf}
    \caption{A real case predicted by Meta-Llama-3-8B-Instruct with few-shots CoT on the coin flip dataset. 
    The \textcolor{purple}{purple} part is an example of input-output pairs given by user.
    The segment highlighted in \textcolor{skyblue}{blue} represents the correct output of the model. 
    The \textcolor{crimson}{red} part shows that the model starts to reason in the wrong direction without control, 
    while the \textcolor{seagreen}{green} portion indicates the model reason in the correct direction after adding control.}
    \label{fig:few_shot_case_llama3_coin_flip}
\end{figure*}

==> tables/case_strategyqa_few.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/case_strategyqa_few.pdf}
    \caption{A real case predicted by Mistral-7B-Instruct-v0.2 with few-shots CoT on the strategyQA dataset. 
    The \textcolor{purple}{purple} part is an example of input-output pairs given by user.
    The segment highlighted in \textcolor{skyblue}{blue} represents the correct output of the model. 
    The \textcolor{crimson}{red} part shows that the model starts to reason in the wrong direction without control, 
    while the \textcolor{seagreen}{green} portion indicates the model reason in the correct direction after adding control.}
    \label{fig:case_strategyqa_few}
\end{figure*}

==> tables/commonsense_reasoning_result_table.tex <==
\begin{table}[ht]
\centering
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{lcc}
\hline
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Commonsense Reasoning} \\ \cline{2-3} 
 & StrategyQA & CSQA \\ \hline
\multicolumn{3}{c}{zero-shot CoT} \\ \hline
Mistral-7B-instruct & 63.01 / \textbf{63.97} & 67.57 / \textbf{67.98} \\
LLaMA-2-7B-chat & 62.66 / \textbf{63.49} & 55.45 / \textbf{56.59} \\
LLaMA-3-8B-instruct & 67.42 / \textbf{68.03} & \textbf{45.29} / 44.39 \\ 
Avg. & 64.36 / 65.16 (\textbf{0.80↑}) & 56.10 / 56.32 (\textbf{0.22↑}) \\ \hline
\multicolumn{3}{c}{few-shot CoT} \\ \hline
Mistral-7B-instruct & 63.49 / \textbf{65.55} & 52.83 / \textbf{54.87} \\
LLaMA-2-7B-chat & 55.63 / \textbf{55.72} & 55.61 / \textbf{58.56} \\
LLaMA-3-8B-instruct & 66.38 / \textbf{68.47} & 67.24 / \textbf{68.47} \\
Avg. & 61.83 / 63.25 (\textbf{1.42↑}) & 58.56 / 60.63 (\textbf{2.07↑}) \\ \hline
\end{tabular}}
\caption{Results on the Commonsense Reasoning task for different models. \label{tab:commonsense_result}}
\vspace{-10pt}
\end{table}

==> tables/control_ag.tex <==
\begin{algorithm}[b]
   \caption{Control Representations\label{alg:control}}
    \KwIn{Query $x$, 
    reading vector $v$, 
    control layers $L$, 
    % coeff $c$,
    model $\mathcal{M}_{\theta}$}
    \KwOut{Model's logits after control}

    \tcp{get the representations of $x$}
    $H \gets Rep(x,\mathcal{M}_{\theta})$ 

    \For{$layer$ \textbf{in} $\mathcal{M}_{\theta}$}{
    \If{$layer$ \textbf{in} $L$}{
            $H[layer] \gets H[layer] + v[layer]$ \label{line:addv}
        }
        % $h \gets \text{layer}(h)$
    }
    \tcp{transform $H$ into the logits of model}
    $logits \gets \text{trans\_into\_logits}(H)$
    
    \textbf{return} $logits$
\end{algorithm}

==> tables/coterror_example.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.90\textwidth]{figures/coterror_example.pdf}
    \caption{
    An example illustrating the sensitivity of LLaMA-2-7B-chat
    % \footnote{\url{https://huggingface.co/meta-llama/Llama-2-7b-chat-hf}}
    in the one-shot scenario. 
    The parts highlighted in \textcolor{springgreen}{\textbf{green}} are the instruction and reasoning path.
    The key difference between the two input-output pairs is highlighted in \textcolor{skyblue}{\textbf{blue}}: The example in the first row has a final answer of ``yes'', while the example in the second row has a final answer of ``no''. We can find that the final output of the model tends to \textit{match} the example, even if the example's result is incorrect. The model adjusts its reasoning steps (highlighted in \textcolor{salmon}{\textbf{red}}) to achieve this consistency.} 
    \vspace{-3.1ex}
    \label{fig:coterrorexample}
\end{figure*}


==> tables/fig1.tex <==
\begin{figure*}[t]
    \centering
    \vspace{-3.7ex}    \includegraphics[width=0.79\linewidth]{figures/cot_framework.pdf}
    \caption{Our CoT explanation framework based on Hopfieldian view.
    \syadd{LLM learned latent (both concrete and abstract) concepts from pertaining documents. These concepts might pertain to specific names or domains, such as ``medical'' or ``climate change''. They could also represent more abstract notions derived from document-level modeling, such as ``positive language'', ``careful reasoning'', or ``affirmative expression''. During the reasoning process, zero-shot or few-shot prompts serve as stimuli for the LLM, inducing the activation of specific concepts. These activated concepts collectively determine the final action of this model. However, directly extracting activated concepts would consume a tremendous amount of computational resources, and individual concepts alone cannot determine the model's overall action. Therefore, we use representations to denote the activation of concepts when the model is stimulated.}\syinline{change the figure to follow this, it's not clear}}
    \vspace{-3.7ex} 
    \label{fig:framework}
\end{figure*}


==> tables/fig2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/LAT.pdf}
    \caption{The pipeline of LAT. \warn{unfinished DO WE NEED THIS FIGURE..?}}
    \label{fig:lat}
\end{figure}

==> tables/framework_example.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\linewidth]
    {figures/framework_example}
    \caption{An example of Presentation of Thought (RoT)}
    \label{fig:rotframework_hidden}
\end{figure*}


==> tables/main_result_ml.tex <==
\begin{table}[]
\centering
\begingroup
\renewcommand{\arraystretch}{1.2}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{lcccccc}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{Arithmetic} & \multicolumn{2}{c}{Commonsense} & \multicolumn{2}{c}{Symbolic} \\ \cline{2-7} 
\multicolumn{1}{c}{} & GSM8K & SVAMP & CSQA & StrategyQA & Coin Flip & Random Letter \\ \hline
\multicolumn{7}{c}{Llama2-7B-chat} \\ \hline
Base & 26.00 & {54.00} & {47.75} & {63.62} & 44.80 & 20.33 \\
\hspace{4pt} + CoT$_Z$ & \textcolor{Green}{26.31} & \textcolor{Red}{46.00} & \textcolor{Red}{43.41} & \textcolor{Red}{62.05} & \textcolor{Green}{52.75} & \textcolor{Green}{24.33} \\
\vspace{3pt}
\hspace{1.5pt} + RoT$_Z$ & \textcolor{Green}{26.23} & \textcolor{Green}{54.33} & \textcolor{Green}{48.24} & \textcolor{Red}{63.54} & \textcolor{Green}{45.45} & \textcolor{Green}{20.67} \\ \hdashline
Base & {26.00} & {54.00} & 47.75 & {63.62} & 44.80 & {20.33} \\
\hspace{4pt} + CoT$_F$ & \textcolor{Red}{4.62} & \textcolor{Red}{38.67} & \textcolor{Green}{53.07} & \textcolor{Red}{59.26} & \textcolor{Green}{47.60} & \textcolor{Green}{31.00} \\ 
\hspace{4pt} + RoT$_F$ & \textcolor{Red}{25.55} & \textcolor{Green}{56.00} & \textcolor{Green}{48.16} & \textcolor{Green}{63.80} & \textcolor{Green}{45.50} & \textcolor{Green}{20.33} \\ \hline
\multicolumn{7}{c}{Llama3-8B-instruct} \\ \hline
Base & 73.31 & 80.67 & {72.65} & 65.07 & 68.90 & {44.00} \\
\hspace{4pt} + CoT$_Z$ & \textcolor{Green}{74.45} & \textcolor{Green}{82.33} & \textcolor{Red}{72.24} & \textcolor{Green}{66.07} & \textcolor{Green}{90.45} & \textcolor{Red}{43.00} \\
\vspace{3pt}
\hspace{1.5pt} + RoT$_Z$ & \textcolor{Green}{74.83} & \textcolor{Green}{83.33} & \textcolor{Green}{72.89} & \textcolor{Green}{65.24} & \textcolor{Green}{76.35} & \textcolor{Green}{47.67} \\ \hdashline
Base & {73.31} & 80.67 & 72.65 & 65.07 & 68.90 & {44.00} \\
\hspace{4pt} + CoT$_F$ & \textcolor{Red}{72.02} & \textcolor{Green}{81.00} & \textcolor{Green}{73.63} & \textcolor{Red}{62.75} & \textcolor{Green}{96.50} & \textcolor{Green}{50.67} \\ 
\hspace{4pt} + RoT$_F$ & \textcolor{Green}{74.37} & \textcolor{Green}{83.67} & \textcolor{Green}{73.30} & \textcolor{Green}{65.94} & \textcolor{Green}{70.30} & \textcolor{Red}{43.66} \\ \hline
\end{tabular}%
}
\caption{Results of RoT and CoT based on different LLMs on a variety of reasoning tasks. 
\textcolor{Green}{Green} indicates an equal or improved accuracy compared to the Base method, while \textcolor{Red}{Red} indicates an accuracy decrease. 
It can be observed that, compared to CoT prompting, RoT achieves more consistent accuracy improvements across a variety of tasks.
}
\label{tab:cotvsrot}
\endgroup
\end{table}


\begin{table}[]
\centering
\begingroup
\renewcommand{\arraystretch}{1.2}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{lcccccc}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{Arithmetic} & \multicolumn{2}{c}{Commonsense} & \multicolumn{2}{c}{Symbolic} \\ \cline{2-7} 
\multicolumn{1}{c}{} & GSM8K & SVAMP & CSQA & StrategyQA & Coin Flip & Random Letter \\ \hline
\multicolumn{7}{c}{Llama2-7B-chat} \\ \hline
CoT$_Z$ & 5.46 & 11.34 & 6.54 & 6.04 & 8.80 & 14.00 \\
RoT$_Z$ & \textbf{3.02} & \textbf{1.32} & \textbf{1.64} & \textbf{0.70} & \textbf{0.30} & \textbf{0.68} \\ \hdashline
CoT$_F$ & 2.88 & 23.94 & 17.52 & 4.80 & 6.90 & 24.66 \\ 
RoT$_F$ & \textbf{0.32} & \textbf{4.00} & \textbf{0.34} & \textbf{3.94} & \textbf{0.30} & \textbf{0.00} \\ \hline
\multicolumn{7}{c}{Llama3-8B-instruct} \\ \hline
CoT$_Z$ & 33.36 & 85.32 & 2.94 & 5.94 & \textbf{13.80} & 18.66 \\
RoT$_Z$ & \textbf{2.58} & \textbf{2.66} & \textbf{0.82} & \textbf{1.14} & 16.40 & \textbf{11.34} \\ \hdashline
CoT$_F$ & 11.98 & \textbf{2.66} & 14.74 & 9.44 & 3.80 & 4.68 \\ 
RoT$_F$ & \textbf{0.90} & 2.68 & \textbf{0.98} & \textbf{0.78} & \textbf{2.20} & \textbf{3.32} \\ \hline
\end{tabular}%
}
\caption{\lijie{$\Delta$ = after perturbation - before perturbation.} The robust results of our approach and different general baselines with CoT on each task. Bold text indicates optimal results in a single dataset. \llinline{Since few-shot deleted an experiment, this table needs to be rewritten. }}
\label{tab:robust}
\endgroup
\end{table}

==> tables/nnrepresentation_figure.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{figures/nn_representation.pdf}
    \caption{nn\_rep~\warn{Todo change to mini page and write a new caption}}
    \label{fig:nnrep}
\end{figure}

==> tables/ntrain_choice_table.tex <==
\begin{table}[ht]
\centering
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{cccc}
\hline
Dataset & Zero-shot & Few-shots  \\ \hline
GSM8K & 128 & 512 \\
SVAMP & 512 & 256  \\
StrategyQA & 512 & 256 \\
CSQA & 512 & 256  \\
Coin Flip & 128 & 512 \\
Random Letter & 128 & 128 \\ \hline
\end{tabular}%
}
\caption{The number of reading set sizes in the experiment.}
\label{tab:ntrain_choices}
\end{table}

==> tables/pos_neg_stimuli.tex <==
\begin{tcolorbox}[colback=white!15,colframe=pink!50!black,left=5pt,right=5pt,top=5pt,bottom=5pt]
\emph{positive stimulus} \\
USER: Would a greyhound be able to outrun a greyhound bus? \\
ASSISTANT: Let's think step by step. \\
\\
\emph{negative stimulus} \\
USER: Would a greyhound be able to outrun a greyhound bus? \\
ASSISTANT:
\end{tcolorbox}

==> tables/stimulus_figure.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{figures/stimulu.pdf}
    \caption{stimulu~\warn{Todo: change to mini page and write a new caption}}
    \label{fig:stimulu}
\end{figure}

==> tables/symbolic_reasoning_result.tex <==
\begin{table}[ht]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccc}
\hline
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Symbolic Reasoning} \\ \cline{2-3} 
 & Coin Flip & Random Letter \\ \hline
\multicolumn{3}{c}{zero-shot CoT} \\ \hline
Mistral-7B-instruct & \textbf{50.80} / 48.95 & 18.33 / \textbf{19.66} \\
LLaMA-2-7B-chat & 52.20 / \textbf{55.75} & 17.33 / \textbf{17.66} \\
LLaMA-3-8B-instruct & 90.45 / \textbf{90.55} & 38.00 / \textbf{38.00} \\ 
Avg. & 64.48 / 65.10 (\textbf{0.62↑}) &  24.55 / 25.11 (\textbf{0.56↑}) \\ \hline
\multicolumn{3}{c}{few-shot CoT} \\ \hline
Mistral-7B-instruct & \textbf{78.73} / 78.19 & 33.67 / \textbf{33.67} \\
LLaMA-2-7B-chat & 50.74 / \textbf{50.84} & 29.67 / \textbf{30.00} \\
LLaMA-3-8B-instruct & 77.02 / \textbf{77.59} & 53.67 / \textbf{54.67} \\
Avg. & 68.83 / 68.87 (\textbf{0.04↑}) & 39.00 / 39.45 (\textbf{0.45↑}) \\ \hline
\end{tabular}}
\caption{Results on the Symbolic Reasoning task for different models. \label{tab:symbolic_result}}
\vspace{-10pt}
\end{table}

==> tables/table_answer_cleansing.tex <==
\begin{table}[h]\centering
%\footnotesize
\caption{Detail description of answer cleansing. See \autoref{tab:dataset_description} for the mapping between each datasets and the corresponding answer formats.}
\label{tab:answer_cleansing}
\begin{tabular}{p{0.15\textwidth}p{0.25\textwidth}p{0.40\textwidth}}
%\begin{tabular}{lrrr}
\toprule
Answer \par Format &Answer Cleansing \par Approach &Pseudo Code \par (Example in Pytorch 3.8) \\\midrule \midrule
Number &Pick up the first number encountered in the text. &
\begin{lstlisting}
pred = pred.replace(",", "")
pred = [s for s in re.findall(r'-?\d+\.?\d*', pred)]
pred = pred[0] 
\end{lstlisting}

\\
\midrule

Multiple-Choice &Pick up the first large letter encountered in the text. &
\begin{lstlisting}
pred = re.findall(r'A|B|C|D|E', pred) 
pred = pred[0]
\end{lstlisting}

\\\midrule

Yes or No &Pick up the first "yes" or "no" encountered in the text after removing unnecessary letters. &
\begin{lstlisting}
pred = pred.lower()
pred = re.sub("\"|\'|\n|\.|\s|\:|\,"," ", pred) 
pred = pred.split(" ") 
pred = [i for i in pred if i in ("yes", "no")] 
pred = pred[0]
\end{lstlisting}

\\\midrule

Free Format &Just remove unnecessary letters, such as ".". &
\begin{lstlisting}
pred = re.sub("\"|\'|\n|\.|\s","", pred)
\end{lstlisting}

\\

\bottomrule
\end{tabular}
\end{table}

==> tables/zero_few_control.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/zero_few_control.pdf}
    \caption{A real case predicted by LLaMA-3-8B-instruct with few-shot CoT on the coin flip dataset. 
    The \textcolor{purple}{purple} part is an example of input-output pairs given by user.
    The segment highlighted in \textcolor{skyblue}{blue} represents the correct output of the model. 
    The \textcolor{crimson}{red} part shows that the model starts to reason in the wrong direction without control, 
    while the \textcolor{seagreen}{green} portion indicates the model reason in the correct direction after adding control.}
    \label{fig:zero_few_control}
\vspace{-12pt}
\end{figure*}







